On the maximum energy of non-thermal particles in the primary hotspot of Cygnus A

We study particle acceleration and magnetic field amplification in the primary hotspot in the northwest jet of radiogalaxy Cygnus A. By using the observed flux density at 43 GHz in a well resolved region of this hotspot, we determine the minimum value of the jet density and constrain the magnitude of the magnetic field. We find that a jet with density greater than $5\times 10^{-5}$ cm$^{-3}$ and hotspot magnetic field in the range 50-400 $\mu$G are required to explain the synchrotron emission at 43 GHz. The upper-energy cut-off in the hotspot synchrotron spectrum is at a frequency < $5\times 10^{14}$ Hz, indicating that the maximum energy of non-thermal electrons accelerated at the jet reverse shock is $E_{e, \rm max} \sim 0.8$ TeV in a magnetic field of 100 $\mu$G. Based on the condition that the magnetic-turbulence scale length has to be larger than the plasma skin depth, and that the energy density in non-thermal particles cannot violate the limit imposed by the jet kinetic luminosity, we show that $E_{e,\rm max}$ cannot be constrained by synchrotron losses as traditionally assumed. In addition to that, and assuming that the shock is quasi-perpendicular, we show that non-resonant hybrid instabilities generated by the streaming of cosmic rays with energy $E_{e, \rm max}$ can grow fast enough to amplify the jet magnetic field up to 50-400 $\mu$G and accelerate particles up to the maximum energy $E_{e, \rm max}$ observed in the Cygnus A primary hotspot.

==> biblio_CRs <==
@ARTICLE{Mixed_Ne,
   author = {{Giannios}, D. and {Spitkovsky}, A.},
    title = "{Signatures of a Maxwellian component in shock-accelerated electrons in GRBs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0905.1970},
 primaryClass = "astro-ph.HE",
 keywords = {acceleration of particles , radiation mechanisms: general , gamma-rays: bursts},
     year = 2009,
    month = nov,
   volume = 400,
    pages = {330-336},
      doi = {10.1111/j.1365-2966.2009.15454.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.400..330G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Spitkovsky_08I,
   author = {{Spitkovsky}, A.},
    title = "{On the Structure of Relativistic Collisionless Shocks in Electron-Ion Plasmas}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0706.3126},
 keywords = {Acceleration of Particles, Gamma Rays: Bursts, Magnetic Fields, Plasmas, Shock Waves},
     year = 2008,
    month = jan,
   volume = 673,
    pages = {L39-L42},
      doi = {10.1086/527374},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...673L..39S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Spitkovsky_08II,
   author = {{Spitkovsky}, A.},
    title = "{Particle Acceleration in Relativistic Collisionless Shocks: Fermi Process at Last?}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0802.3216},
 keywords = {Acceleration of Particles, Gamma Rays: Bursts, Shock Waves},
     year = 2008,
    month = jul,
   volume = 682,
    pages = {L5-L8},
      doi = {10.1086/590248},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...682L...5S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Erlund_TwoShocks,
   author = {{Erlund}, M.~C. and {Fabian}, A.~C. and {Blundell}, K.~M. and 
	{Crawford}, C.~S. and {Hirst}, P.},
    title = "{Two types of shock in the hotspot of the giant quasar 4C74.26: a high-resolution comparison from Chandra, Gemini and MERLIN}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1001.1063},
 primaryClass = "astro-ph.CO",
 keywords = {quasars: individual: 4C74.26, X-rays: general},
     year = 2010,
    month = may,
   volume = 404,
    pages = {629-640},
      doi = {10.1111/j.1365-2966.2010.16304.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.404..629E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Erlund_Xrays,
   author = {{Erlund}, M.~C. and {Fabian}, A.~C. and {Blundell}, K.~M. and 
	{Moss}, C. and {Ballantyne}, D.~R.},
    title = "{The luminous X-ray hotspot in 4C74.26: synchrotron or inverse-Compton emission?}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0705.1339},
 keywords = {quasars: individual: 4C74.26, X-rays: general},
     year = 2007,
    month = aug,
   volume = 379,
    pages = {498-506},
      doi = {10.1111/j.1365-2966.2007.11962.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.379..498E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Stage_06,
   author = {{Stage}, M.~D. and {Allen}, G.~E. and {Houck}, J.~C. and {Davis}, J.~E.
	},
    title = "{Cosmic-ray diffusion near the Bohm limit in the Cassiopeia A supernova remnant}",
  journal = {Nature Physics},
   eprint = {astro-ph/0608401},
     year = 2006,
    month = sep,
   volume = 2,
    pages = {614-619},
      doi = {10.1038/nphys391},
   adsurl = {http://adsabs.harvard.edu/abs/2006NatPh...2..614S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Brian_14,
   author = {{Reville}, B. and {Bell}, A.~R.},
    title = "{On the maximum energy of shock-accelerated cosmic rays at ultra-relativistic shocks}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1401.2803},
 primaryClass = "astro-ph.HE",
 keywords = {acceleration of particles, instabilities, plasmas, shock waves, cosmic rays},
     year = 2014,
    month = apr,
   volume = 439,
    pages = {2050-2059},
      doi = {10.1093/mnras/stu088},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.439.2050R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sironi_11,
   author = {{Sironi}, L. and {Spitkovsky}, A.},
    title = "{Particle Acceleration in Relativistic Magnetized Collisionless Electron-Ion Shocks}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1009.0024},
 primaryClass = "astro-ph.HE",
 keywords = {acceleration of particles, cosmic rays, galaxies: jets, gamma-ray burst: general, shock waves},
     year = 2011,
    month = jan,
   volume = 726,
      eid = {75},
    pages = {75},
      doi = {10.1088/0004-637X/726/2/75},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...726...75S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sironi_13,
   author = {{Sironi}, L. and {Spitkovsky}, A. and {Arons}, J.},
    title = "{The Maximum Energy of Accelerated Particles in Relativistic Collisionless Shocks}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1301.5333},
 primaryClass = "astro-ph.HE",
 keywords = {acceleration of particles, cosmic rays, gamma-ray burst: general, pulsars: general, radiation mechanisms: non-thermal, shock waves},
     year = 2013,
    month = jul,
   volume = 771,
      eid = {54},
    pages = {54},
      doi = {10.1088/0004-637X/771/1/54},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...771...54S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kirk_87,
   author = {{Kirk}, J.~G. and {Schneider}, P.},
    title = "{On the acceleration of charged particles at relativistic shock fronts}",
  journal = {\apj},
 keywords = {Charged Particles, Computational Astrophysics, Particle Acceleration, Relativistic Velocity, Shock Fronts, Approximation, Cosmic Rays, Kinetic Equations, Particle Diffusion, Radio Sources (Astronomy), Solar Flares},
     year = 1987,
    month = apr,
   volume = 315,
    pages = {425-433},
      doi = {10.1086/165147},
   adsurl = {http://adsabs.harvard.edu/abs/1987ApJ...315..425K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bell_04,
   author = {{Bell}, A.~R.},
    title = "{Turbulent amplification of magnetic field and diffusive shock acceleration of cosmic rays}",
  journal = {\mnras},
 keywords = {acceleration of particles, magnetic fields, plasmas, shock waves, turbulence, cosmic rays},
     year = 2004,
    month = sep,
   volume = 353,
    pages = {550-558},
      doi = {10.1111/j.1365-2966.2004.08097.x},
   adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.353..550B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sources,
   author = {{Orienti}, M. and {Prieto}, M.~A. and {Brunetti}, G. and {Mack}, K.-H. and 
	{Massaro}, F. and {Harris}, D.~E.},
    title = "{Complex particle acceleration processes in the hotspots of 3C 105 and 3C 445}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1109.4895},
 primaryClass = "astro-ph.CO",
 keywords = {acceleration of particles, radiation mechanisms: non-thermal, radio continuum: galaxies},
     year = 2012,
    month = jan,
   volume = 419,
    pages = {2338-2348},
      doi = {10.1111/j.1365-2966.2011.19882.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.419.2338O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bell_rev_14,
   author = {{Bell}, A.~R.},
    title = "{Particle Acceleration by Shocks in Supernova Remnants}",
  journal = {Brazilian Journal of Physics},
archivePrefix = "arXiv",
   eprint = {1311.5779},
 primaryClass = "astro-ph.HE",
 keywords = {Cosmic rays, Particle acceleration, Magnetic field, Supernova remnants},
     year = 2014,
    month = oct,
   volume = 44,
    pages = {415-425},
      doi = {10.1007/s13538-014-0219-5},
   adsurl = {http://adsabs.harvard.edu/abs/2014BrJPh..44..415B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{3c273-Natur,
   author = {{Meisenheimer}, K. and {Heavens}, A.~F.},
    title = "{Particle acceleration in the hotspot of the jet of quasar 3C273}",
  journal = {\nat},
 keywords = {Astronomical Spectroscopy, Electron Acceleration, Quasars, Radio Jets (Astronomy), Synchrotron Radiation, Emission Spectra, Interstellar Magnetic Fields, Radio Spectra, Shock Waves, Spectrum Analysis},
     year = 1986,
    month = oct,
   volume = 323,
    pages = {419-422},
      doi = {10.1038/323419a0},
   adsurl = {http://adsabs.harvard.edu/abs/1986Natur.323..419M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Klara_review,
   author = {{Schure}, K.~M. and {Bell}, A.~R. and {O'C Drury}, L. and {Bykov}, A.~M.
	},
    title = "{Diffusive Shock Acceleration and Magnetic Field Amplification}",
  journal = {\ssr},
archivePrefix = "arXiv",
   eprint = {1203.1637},
 primaryClass = "astro-ph.HE",
 keywords = {Cosmic rays, Instabilities, Acceleration of particles},
     year = 2012,
    month = nov,
   volume = 173,
    pages = {491-519},
      doi = {10.1007/s11214-012-9871-7},
   adsurl = {http://adsabs.harvard.edu/abs/2012SSRv..173..491S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Meisenheimer_89,
   author = {{Meisenheimer}, K. and {Roser}, H.-J. and {Hiltner}, P.~R. and 
	{Yates}, M.~G. and {Longair}, M.~S. and {Chini}, R. and {Perley}, R.~A.
	},
    title = "{The synchrotron spectra of radio hot spots}",
  journal = {\aap},
 keywords = {Astronomical Spectroscopy, Radio Galaxies, Synchrotron Radiation, Emission Spectra, Infrared Photometry, Particle Acceleration, Radio Jets (Astronomy)},
     year = 1989,
    month = jul,
   volume = 219,
    pages = {63-86},
   adsurl = {http://adsabs.harvard.edu/abs/1989A%26A...219...63M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Vink-Laming,
   author = {{Vink}, J. and {Laming}, J.~M.},
    title = "{On the Magnetic Fields and Particle Acceleration in Cassiopeia A}",
  journal = {\apj},
   eprint = {astro-ph/0210669},
 keywords = {Acceleration of Particles, Gamma Rays: Observations- ISM: Individual: Name: Cassiopeia A, Magnetic Fields- Shock Waves, ISM: Supernova Remnants},
     year = 2003,
    month = feb,
   volume = 584,
    pages = {758-769},
      doi = {10.1086/345832},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...584..758V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{lemoine-pelletier-10,
   author = {{Lemoine}, M. and {Pelletier}, G.},
    title = "{On electromagnetic instabilities at ultra-relativistic shock waves}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0904.2657},
 primaryClass = "astro-ph.HE",
 keywords = {acceleration of particles, shock waves, cosmic rays},
     year = 2010,
    month = feb,
   volume = 402,
    pages = {321-334},
      doi = {10.1111/j.1365-2966.2009.15869.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.402..321L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lemoine-Weibel-14,
   author = {{Lemoine}, M.},
    title = "{Non-linear collisionless damping of Weibel turbulence in relativistic blast waves}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1410.0146},
 primaryClass = "physics.plasm-ph",
 keywords = {Physics - Plasma Physics, Astrophysics - High Energy Astrophysical Phenomena},
     year = 2014,
    month = oct,
   adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1410.0146L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Berezhko-03,
   author = {{Berezhko}, E.~G. and {Ksenofontov}, L.~T. and {V{\"o}lk}, H.~J.
	},
    title = "{Confirmation of strong magnetic field amplification and nuclear cosmic ray acceleration in SN 1006}",
  journal = {\aap},
   eprint = {astro-ph/0310862},
 keywords = {ISM: cosmic rays, supernova remnants, individual: SN 1006},
     year = 2003,
    month = dec,
   volume = 412,
    pages = {L11-L14},
      doi = {10.1051/0004-6361:20031667},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...412L..11B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{B_equip,
   author = {{Godfrey}, L.~E.~H. and {Shabala}, S.~S.},
    title = "{AGN Jet Kinetic Power and the Energy Budget of Radio Galaxy Lobes}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1301.3499},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: active},
     year = 2013,
    month = apr,
   volume = 767,
      eid = {12},
    pages = {12},
      doi = {10.1088/0004-637X/767/1/12},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...767...12G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{FR,
   author = {{Fanaroff}, B.~L. and {Riley}, J.~M.},
    title = "{The morphology of extragalactic radio sources of high and low luminosity}",
  journal = {\mnras},
     year = 1974,
    month = may,
   volume = 167,
    pages = {31P-36P},
   adsurl = {http://adsabs.harvard.edu/abs/1974MNRAS.167P..31F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wilson_00,
   author = {{Wilson}, A.~S. and {Young}, A.~J. and {Shopbell}, P.~L.},
    title = "{Chandra Observations of Cygnus A: Magnetic Field Strengths in the Hot Spots of a Radio Galaxy}",
  journal = {\apjl},
   eprint = {astro-ph/0009308},
 keywords = {Galaxies: Active, Galaxies: Individual: Name: Cygnus A, Galaxies: Jets, Galaxies: Nuclei, Magnetic Fields, X-Rays: Galaxies},
     year = 2000,
    month = nov,
   volume = 544,
    pages = {L27-L30},
      doi = {10.1086/317293},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...544L..27W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Nilsson_97,
   author = {{Nilsson}, K. and {Valtonen}, M.~J. and {Jones}, L.~R. and {Saslaw}, W.~C. and 
	{Lehto}, H.~J.},
    title = "{Optical emission in the radio lobes of Cygnus A.}",
  journal = {\aap},
 keywords = {GALAXIES: ACTIVE, GALAXIES: INDIVIDUAL: CYGNUS A, RADIO CONTINUUM: GALAXIES, ACCRETION, ACCRETION DISKS},
     year = 1997,
    month = aug,
   volume = 324,
    pages = {888-898},
   adsurl = {http://adsabs.harvard.edu/abs/1997A%26A...324..888N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Stawarz_07,
   author = {{Stawarz}, {\L}. and {Cheung}, C.~C. and {Harris}, D.~E. and 
	{Ostrowski}, M.},
    title = "{The Electron Energy Distribution in the Hotspots of Cygnus A: Filling the Gap with the Spitzer Space Telescope}",
  journal = {\apj},
   eprint = {astro-ph/0701568},
 keywords = {Acceleration of Particles, Galaxies: Individual: Name: Cygnus A, Galaxies: Jets, Radiation Mechanisms: Nonthermal},
     year = 2007,
    month = jun,
   volume = 662,
    pages = {213-223},
      doi = {10.1086/517966},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...662..213S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Carilli_99,
   author = {{Carilli}, C.~L. and {Kurk}, J.~D. and {van der Werf}, P.~P. and 
	{Perley}, R.~A. and {Miley}, G.~K.},
    title = "{High-Resolution Millimeter and Infrared Observations of the Hot Spots of Cygnus A}",
  journal = {\aj},
 keywords = {GALAXIES: ACTIVE, GALAXIES: INDIVIDUAL (CYGNUS A), GALAXIES: JETS, INFRARED RADIATION, PHYSICAL DATA AND PROCESSES},
     year = 1999,
    month = dec,
   volume = 118,
    pages = {2581-2591},
      doi = {10.1086/301137},
   adsurl = {http://adsabs.harvard.edu/abs/1999AJ....118.2581C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Carilli_91,
   author = {{Carilli}, C.~L. and {Perley}, R.~A. and {Dreher}, J.~W. and 
	{Leahy}, J.~P.},
    title = "{Multifrequency radio observations of Cygnus A - Spectral aging in powerful radio galaxies}",
  journal = {\apj},
 keywords = {Galactic Evolution, Radio Astronomy, Radio Galaxies, Radio Jets (Astronomy), Astronomical Models, Cygnus Constellation, Emission Spectra, Particle Acceleration, Radio Spectra, Synchrotron Radiation},
     year = 1991,
    month = dec,
   volume = 383,
    pages = {554-573},
      doi = {10.1086/170813},
   adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...383..554C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pyrzas_15,
   author = {{Pyrzas}, S. and {Steenbrugge}, K.~C. and {Blundell}, K.~M.},
    title = "{Multiwavelength study of Cygnus A. V. The hotspots in the lobe}",
  journal = {\aap},
 keywords = {galaxies: active, galaxies: individual: Cygnus A, galaxies: jets},
     year = 2015,
    month = feb,
   volume = 574,
      eid = {A30},
    pages = {A30},
      doi = {10.1051/0004-6361/201425061},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...574A..30P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wright_04,
   author = {{Wright}, M.~C.~H. and {Birkinshaw}, M.},
    title = "{The Hot Spots of Cygnus A at 230 GHz}",
  journal = {\apj},
 keywords = {Galaxies: Active, Galaxies: Individual: Name: Cygnus A, Radio Continuum: Galaxies, Techniques: Interferometric},
     year = 2004,
    month = oct,
   volume = 614,
    pages = {115-121},
      doi = {10.1086/423483},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...614..115W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{4c7426,
   author = {{Araudo}, A.~T. and {Bell}, A.~R. and {Blundell}, K.~M.},
    title = "{Particle Acceleration and Magnetic Field Amplification in the Jets of 4C74.26}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1505.02210},
 primaryClass = "astro-ph.HE",
 keywords = {acceleration of particles, galaxies: active, galaxies: jets, quasars: individual: 4C74.26, radiation mechanisms: non-thermal, shock waves},
     year = 2015,
    month = jun,
   volume = 806,
      eid = {243},
    pages = {243},
      doi = {10.1088/0004-637X/806/2/243},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...806..243A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kardashev_62,
   author = {{Kardashev}, N.~S.},
    title = "{Nonstationarity of Spectra of Young Sources of Nonthermal Radio Emission}",
  journal = {\sovast},
     year = 1962,
    month = dec,
   volume = 6,
    pages = {317},
   adsurl = {http://adsabs.harvard.edu/abs/1962SvA.....6..317K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Steenbrugge_08,
   author = {{Steenbrugge}, K.~C. and {Blundell}, K.~M.},
    title = "{Multiwavelength study of CygnusA - I. Precession and slow jet speeds from radio observations}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0805.2169},
 keywords = {galaxies: active , galaxies: individual: CygnusA , galaxies: jets},
     year = 2008,
    month = aug,
   volume = 388,
    pages = {1457-1464},
      doi = {10.1111/j.1365-2966.2007.12665.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.388.1457S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{polarization,
   author = {{Dreher}, J.~W. and {Carilli}, C.~L. and {Perley}, R.~A.},
    title = "{The Faraday rotation of Cygnus A - Magnetic fields in cluster gas}",
  journal = {\apj},
 keywords = {Cosmic Gases, Faraday Effect, Galactic Clusters, Intergalactic Media, Interstellar Magnetic Fields, Astronomical Maps, Polarization (Waves), Radio Emission},
     year = 1987,
    month = may,
   volume = 316,
    pages = {611-625},
      doi = {10.1086/165229},
   adsurl = {http://adsabs.harvard.edu/abs/1987ApJ...316..611D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hillas,
   author = {{Hillas}, A.~M.},
    title = "{The Origin of Ultra-High-Energy Cosmic Rays}",
  journal = {\araa},
     year = 1984,
   volume = 22,
    pages = {425-444},
      doi = {10.1146/annurev.aa.22.090184.002233},
   adsurl = {http://adsabs.harvard.edu/abs/1984ARA%26A..22..425H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Croston_09,
   author = {{Croston}, J.~H. and {Kraft}, R.~P. and {Hardcastle}, M.~J. and 
	{Birkinshaw}, M. and {Worrall}, D.~M. and {Nulsen}, P.~E.~J. and 
	{Penna}, R.~F. and {Sivakoff}, G.~R. and {Jord{\'a}n}, A. and 
	{Brassington}, N.~J. and {Evans}, D.~A. and {Forman}, W.~R. and 
	{Gilfanov}, M. and {Goodger}, J.~L. and {Harris}, W.~E. and 
	{Jones}, C. and {Juett}, A.~M. and {Murray}, S.~S. and {Raychaudhury}, S. and 
	{Sarazin}, C.~L. and {Voss}, R. and {Woodley}, K.~A.},
    title = "{High-energy particle acceleration at the radio-lobe shock of Centaurus A}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0901.1346},
 primaryClass = "astro-ph.HE",
 keywords = {shock waves , galaxies: active , galaxies: elliptical and lenticular: cD , galaxies: individual: Cen A , radio continuum: galaxies , X-rays: galaxies},
     year = 2009,
    month = jun,
   volume = 395,
    pages = {1999-2012},
      doi = {10.1111/j.1365-2966.2009.14715.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.395.1999C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mack_09,
   author = {{Mack}, K.-H. and {Prieto}, M.~A. and {Brunetti}, G. and {Orienti}, M.
	},
    title = "{Near-infrared/optical counterparts of hotspots in radio galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0810.3764},
 keywords = {galaxies: active , galaxies: jets , radio continuum: galaxies},
     year = 2009,
    month = jan,
   volume = 392,
    pages = {705-717},
      doi = {10.1111/j.1365-2966.2008.14081.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.392..705M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Blasi_Amato_12,
   author = {{Blasi}, P. and {Amato}, E.},
    title = "{Diffusive propagation of cosmic rays from supernova remnants in the Galaxy. II: anisotropy}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1105.4529},
 primaryClass = "astro-ph.HE",
     year = 2012,
    month = jan,
   volume = 1,
      eid = {011},
    pages = {11},
      doi = {10.1088/1475-7516/2012/01/011},
   adsurl = {http://adsabs.harvard.edu/abs/2012JCAP...01..011B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tingay_08,
   author = {{Tingay}, S.~J. and {Lenc}, E. and {Brunetti}, G. and {Bondi}, M.
	},
    title = "{A High Resolution View of the Jet Termination Shock in a Hot Spot of the Nearby Radio Galaxy Pictor A: Implications for X-Ray Models of Radio Galaxy Hot Spots}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {0810.0321},
 keywords = {galaxies: active, galaxies: individual: Pictor A, galaxies: jets, radio continuum: galaxies},
     year = 2008,
    month = dec,
   volume = 136,
    pages = {2473-2482},
      doi = {10.1088/0004-6256/136/6/2473},
   adsurl = {http://adsabs.harvard.edu/abs/2008AJ....136.2473T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hardcastle_98,
   author = {{Hardcastle}, M.~J. and {Alexander}, P. and {Pooley}, G.~G. and 
	{Riley}, J.~M.},
    title = "{FRII radio galaxies with z{\lt}0.3 - I. Properties of jets, cores and hotspots}",
  journal = {\mnras},
   eprint = {astro-ph/9801179},
 keywords = {GALAXIES: ACTIVE, GALAXIES: JETS, RADIO CONTINUUM: GALAXIES},
     year = 1998,
    month = may,
   volume = 296,
    pages = {445-462},
      doi = {10.1046/j.1365-8711.1998.01480.x},
   adsurl = {http://adsabs.harvard.edu/abs/1998MNRAS.296..445H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hardcastle_97,
   author = {{Hardcastle}, M.~J. and {Alexander}, P. and {Pooley}, G.~G. and 
	{Riley}, J.~M.},
    title = "{High-resolution observations at 3.6cm of seventeen FRII radio galaxies with 0.15{\lt}z{\lt}0.30}",
  journal = {\mnras},
 keywords = {GALAXIES: ACTIVE, GALAXIES: JETS, RADIO CONTINUUM: GALAXIES},
     year = 1997,
    month = jul,
   volume = 288,
    pages = {859-890},
   adsurl = {http://adsabs.harvard.edu/abs/1997MNRAS.288..859H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Leahy_97,
   author = {{Leahy}, J.~P. and {Black}, A.~R.~S. and {Dennett-Thorpe}, J. and 
	{Hardcastle}, M.~J. and {Komissarov}, S. and {Perley}, R.~A. and 
	{Riley}, J.~M. and {Scheuer}, P.~A.~G.},
    title = "{A study of FRII radio galaxies with z{\lt}0.15 - II. High-resolution maps of 11 sources at 3.6 CM}",
  journal = {\mnras},
 keywords = {MAGNETIC FIELDS, POLARIZATION, GALAXIES: ACTIVE, GALAXIES: JETS, RADIO CONTINUUM: GALAXIES},
     year = 1997,
    month = oct,
   volume = 291,
    pages = {20-53},
   adsurl = {http://adsabs.harvard.edu/abs/1997MNRAS.291...20L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Krause_12,
   author = {{Krause}, M. and {Alexander}, P. and {Riley}, J. and {Hopton}, D.
	},
    title = "{A new connection between the jet opening angle and the large-scale morphology of extragalactic radio sources}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1206.1778},
 keywords = {methods: numerical, galaxies: jets, radio continuum: galaxies},
     year = 2012,
    month = dec,
   volume = 427,
    pages = {3196-3208},
      doi = {10.1111/j.1365-2966.2012.21645.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.427.3196K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Monceau-Baroux-12,
   author = {{Monceau-Baroux}, R. and {Keppens}, R. and {Meliani}, Z.},
    title = "{The effect of angular opening on the dynamics of relativistic hydro jets}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1211.1590},
 primaryClass = "astro-ph.HE",
 keywords = {hydrodynamics, relativistic processes, galaxies: jets},
     year = 2012,
    month = sep,
   volume = 545,
      eid = {A62},
    pages = {A62},
      doi = {10.1051/0004-6361/201219308},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...545A..62M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Komissarov_Falle_98,
   author = {{Komissarov}, S.~S. and {Falle}, S.~A.~E.~G.},
    title = "{The large-scale structure of FR-II radio sources}",
  journal = {\mnras},
 keywords = {HYDRODYNAMICS, RADIATION MECHANISMS: NON-THERMAL, RELATIVITY, GALAXIES: JETS},
     year = 1998,
    month = jul,
   volume = 297,
    pages = {1087-1108},
      doi = {10.1046/j.1365-8711.1998.01547.x},
   adsurl = {http://adsabs.harvard.edu/abs/1998MNRAS.297.1087K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Perlman_10,
   author = {{Perlman}, E.~S. and {Georganopoulos}, M. and {May}, E.~M. and 
	{Kazanas}, D.},
    title = "{Chandra Observations of the Radio Galaxy 3C 445 and the Hot Spot X-Ray Emission Mechanism}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0910.3021},
 primaryClass = "astro-ph.HE",
 keywords = {galaxies: active, galaxies: individual: 3C 445, galaxies: jets, radio continuum: galaxies, X-rays: galaxies},
     year = 2010,
    month = jan,
   volume = 708,
    pages = {1-8},
      doi = {10.1088/0004-637X/708/1/1},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...708....1P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hardcastle_07,
   author = {{Hardcastle}, M.~J. and {Croston}, J.~H. and {Kraft}, R.~P.},
    title = "{A Chandra Study of Particle Acceleration in the Multiple Hot Spots of Nearby Radio Galaxies}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0707.2865},
 keywords = {Galaxies: Active, X-Rays: Galaxies},
     year = 2007,
    month = nov,
   volume = 669,
    pages = {893-904},
      doi = {10.1086/521696},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...669..893H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hardcastle_04,
   author = {{Hardcastle}, M.~J. and {Harris}, D.~E. and {Worrall}, D.~M. and 
	{Birkinshaw}, M.},
    title = "{The Origins of X-Ray Emission from the Hot Spots of FR II Radio Sources}",
  journal = {\apj},
   eprint = {astro-ph/0405516},
 keywords = {Galaxies: Active, Galaxies: Quasars: General, Radiation Mechanisms: Nonthermal, X-Rays: Galaxies},
     year = 2004,
    month = sep,
   volume = 612,
    pages = {729-748},
      doi = {10.1086/422808},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...612..729H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{3C445_02Sci,
   author = {{Prieto}, M.~A. and {Brunetti}, G. and {Mack}, K.-H.},
    title = "{Particle Accelerators in the Hot Spots of Radio Galaxy 3C 445, Imaged with the VLT}",
  journal = {Science},
   eprint = {astro-ph/0210304},
     year = 2002,
    month = oct,
   volume = 298,
    pages = {193-195},
      doi = {10.1126/science.1075990},
   adsurl = {http://adsabs.harvard.edu/abs/2002Sci...298..193P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Werner_12,
   author = {{Werner}, M.~W. and {Murphy}, D.~W. and {Livingston}, J.~H. and 
	{Gorjian}, V. and {Jones}, D.~L. and {Meier}, D.~L. and {Lawrence}, C.~R.
	},
    title = "{Spitzer Observations of Hotspots in Radio Lobes}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1209.0810},
 keywords = {acceleration of particles, radiation mechanisms: non-thermal},
     year = 2012,
    month = nov,
   volume = 759,
      eid = {86},
    pages = {86},
      doi = {10.1088/0004-637X/759/2/86},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...759...86W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Zhang_10,
   author = {{Zhang}, J. and {Bai}, J.~M. and {Chen}, L. and {Liang}, E.},
    title = "{X-Ray Radiation Mechanisms and Beaming Effect of Hot Spots and Knots in Active Galactic Nuclear Jets}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0912.2470},
 primaryClass = "astro-ph.HE",
 keywords = {galaxies: jets, magnetic fields, radiation mechanisms: non-thermal, X-rays: galaxies},
     year = 2010,
    month = feb,
   volume = 710,
    pages = {1017-1031},
      doi = {10.1088/0004-637X/710/2/1017},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...710.1017Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chang_08,
   author = {{Chang}, P. and {Spitkovsky}, A. and {Arons}, J.},
    title = "{Long-Term Evolution of Magnetic Turbulence in Relativistic Collisionless Shocks: Electron-Positron Plasmas}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0704.3832},
 keywords = {Gamma Rays: Bursts, Plasmas, Shock Waves, Turbulence},
     year = 2008,
    month = feb,
   volume = 674,
    pages = {378-387},
      doi = {10.1086/524764},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...674..378C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kirk_00,
   author = {{Kirk}, J.~G. and {Guthmann}, A.~W. and {Gallant}, Y.~A. and 
	{Achterberg}, A.},
    title = "{Particle Acceleration at Ultrarelativistic Shocks: An Eigenfunction Method}",
  journal = {\apj},
   eprint = {astro-ph/0005222},
 keywords = {Acceleration of Particles, Galaxies: Jets, Gamma Rays: Bursts, Plasmas, Stars: Pulsars: General, Shock Waves},
     year = 2000,
    month = oct,
   volume = 542,
    pages = {235-242},
      doi = {10.1086/309533},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...542..235K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kraft_05,
   author = {{Kraft}, R.~P. and {Hardcastle}, M.~J. and {Worrall}, D.~M. and 
	{Murray}, S.~S.},
    title = "{A Chandra Study of the Multicomponent X-Ray Emission from the X-shaped Radio Galaxy 3C 403}",
  journal = {\apj},
   eprint = {astro-ph/0501031},
 keywords = {Galaxies: Active, Galaxies: Individual: Alphanumeric: 3C 403, Galaxies: ISM, X-Rays: Galaxies},
     year = 2005,
    month = mar,
   volume = 622,
    pages = {149-159},
      doi = {10.1086/427822},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...622..149K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Achterberg_01,
   author = {{Achterberg}, A. and {Gallant}, Y.~A. and {Kirk}, J.~G. and 
	{Guthmann}, A.~W.},
    title = "{Particle acceleration by ultrarelativistic shocks: theory and simulations}",
  journal = {\mnras},
   eprint = {astro-ph/0107530},
 keywords = {ACCELERATION OF PARTICLES, SHOCK WAVES, COSMIC RAYS, GAMMA-RAYS: BURSTS},
     year = 2001,
    month = dec,
   volume = 328,
    pages = {393-408},
      doi = {10.1046/j.1365-8711.2001.04851.x},
   adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.328..393A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Black_92,
   author = {{Black}, A.~R.~S. and {Baum}, S.~A. and {Leahy}, J.~P. and {Perley}, R.~A. and 
	{Riley}, J.~M. and {Scheuer}, P.~A.~G.},
    title = "{A study of FRII radio galaxies with Z less than 0.15. I - High-resolution maps of eight sources at 3.6 CM}",
  journal = {\mnras},
 keywords = {Active Galaxies, Galactic Radio Waves, Radio Galaxies, Radio Jets (Astronomy), Astronomical Maps, Radio Astronomy, Very Large Array (Vla)},
     year = 1992,
    month = may,
   volume = 256,
    pages = {186-208},
   adsurl = {http://adsabs.harvard.edu/abs/1992MNRAS.256..186B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lemoine_15_NonLinear,
   author = {{Lemoine}, M.},
    title = "{Nonlinear collisionless damping of Weibel turbulence in relativistic blast waves}",
  journal = {Journal of Plasma Physics},
archivePrefix = "arXiv",
   eprint = {1410.0146},
 primaryClass = "physics.plasm-ph",
     year = 2015,
    month = jan,
   volume = 81,
   number = 1,
      eid = {455810101},
    pages = {014501},
      doi = {10.1017/S0022377814000920},
   adsurl = {http://adsabs.harvard.edu/abs/2015JPlPh..81a4501L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{theta_jet,
   author = {{Safouris}, V. and {Subrahmanyan}, R. and {Bicknell}, G.~V. and 
	{Saripalli}, L.},
    title = "{PKS B1545-321: bow shocks of a relativistic jet?}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0802.0538},
 keywords = {galaxies: active , galaxies: individual: PKS B1545-321 , galaxies: jets , radio continuum: galaxies},
     year = 2008,
    month = apr,
   volume = 385,
    pages = {2117-2135},
      doi = {10.1111/j.1365-2966.2008.12975.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.385.2117S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Mizuta_04,
   author = {{Mizuta}, A. and {Yamada}, S. and {Takabe}, H.},
    title = "{Propagation and Dynamics of Relativistic Jets}",
  journal = {\apj},
   eprint = {astro-ph/0402355},
 keywords = {Galaxies: Jets, Hydrodynamics, Methods: Numerical, Relativity, Shock Waves},
     year = 2004,
    month = may,
   volume = 606,
    pages = {804-818},
      doi = {10.1086/382779},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...606..804M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Medvedev_05,
   author = {{Medvedev}, M.~V. and {Fiore}, M. and {Fonseca}, R.~A. and {Silva}, L.~O. and 
	{Mori}, W.~B.},
    title = "{Long-Time Evolution of Magnetic Fields in Relativistic Gamma-Ray Burst Shocks}",
  journal = {\apjl},
   eprint = {astro-ph/0409382},
 keywords = {Gamma Rays: Bursts, Magnetic Fields, Shock Waves, ISM: Supernova Remnants},
     year = 2005,
    month = jan,
   volume = 618,
    pages = {L75-L78},
      doi = {10.1086/427921},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...618L..75M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Peer_06,
   author = {{Pe'er}, A. and {Zhang}, B.},
    title = "{Synchrotron Emission in Small-Scale Magnetic Fields as a Possible Explanation for Prompt Emission Spectra of Gamma-Ray Bursts}",
  journal = {\apj},
   eprint = {astro-ph/0605641},
 keywords = {Gamma Rays: Bursts, Gamma Rays: Theory, Magnetic Fields, Plasmas, Radiation Mechanisms: Nonthermal},
     year = 2006,
    month = dec,
   volume = 653,
    pages = {454-461},
      doi = {10.1086/508681},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...653..454P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Scheuer_95,
   author = {{Scheuer}, P.~A.~G.},
    title = "{Lobe Asymmetry and the Expansion Speeds of Radio Sources}",
  journal = {\mnras},
     year = 1995,
    month = nov,
   volume = 277,
    pages = {331},
   adsurl = {http://adsabs.harvard.edu/abs/1995MNRAS.277..331S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lagage-Cesarsky,
   author = {{Lagage}, P.~O. and {Cesarsky}, C.~J.},
    title = "{The maximum energy of cosmic rays accelerated by supernova shocks}",
  journal = {\aap},
 keywords = {Cosmic Rays, Particle Acceleration, Particle Energy, Shock Wave Propagation, Supernovae, Diffusion Coefficient, Magnetohydrodynamic Waves, Milky Way Galaxy, Particle Diffusion},
     year = 1983,
    month = sep,
   volume = 125,
    pages = {249-257},
   adsurl = {http://adsabs.harvard.edu/abs/1983A%26A...125..249L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DeYoung_02,
   author = {{De Young}, D.~S.},
    title = "{Magnetic field amplification in FR II hotspots}",
  journal = {\nar},
     year = 2002,
    month = may,
   volume = 46,
    pages = {393-397},
      doi = {10.1016/S1387-6473(02)00149-5},
   adsurl = {http://adsabs.harvard.edu/abs/2002NewAR..46..393D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Brunetti_03,
   author = {{Brunetti}, G. and {Mack}, K.-H. and {Prieto}, M.~A. and {Varano}, S.
	},
    title = "{In-situ particle acceleration in extragalactic radio hot spots: observations meet expectations}",
  journal = {\mnras},
   eprint = {astro-ph/0309290},
 keywords = {acceleration of particles, radiation mechanisms: non-thermal, shock waves, galaxies: active, galaxies: jets},
     year = 2003,
    month = nov,
   volume = 345,
    pages = {L40-L44},
      doi = {10.1046/j.1365-8711.2003.07185.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.345L..40B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Meisenheimer_IR,
   author = {{Meisenheimer}, K. and {Yates}, M.~G. and {Roeser}, H.-J.},
    title = "{The synchrotron spectra of radio hot spots. II. Infrared imaging.}",
  journal = {\aap},
 keywords = {RADIATION MECHANISM: NON-THERMAL, RADIO CONTINUUM: GALAXIES, GALAXIES: GENERAL},
     year = 1997,
    month = sep,
   volume = 325,
    pages = {57-73},
   adsurl = {http://adsabs.harvard.edu/abs/1997A%26A...325...57M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gruzinov_99,
   author = {{Gruzinov}, A. and {Waxman}, E.},
    title = "{Gamma-Ray Burst Afterglow: Polarization and Analytic Light Curves}",
  journal = {\apj},
   eprint = {astro-ph/9807111},
 keywords = {GAMMA RAYS: BURSTS, POLARIZATION, RADIATION MECHANISMS: NONTHERMAL, SHOCK WAVES, STARS: MAGNETIC FIELDS, Gamma Rays: Bursts, Polarization, Radiation Mechanisms: Nonthermal, Shock Waves, Stars: Magnetic Fields},
     year = 1999,
    month = feb,
   volume = 511,
    pages = {852-861},
      doi = {10.1086/306720},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...511..852G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sironi_rev,
   author = {{Sironi}, L. and {Keshet}, U. and {Lemoine}, M.},
    title = "{Relativistic Shocks: Particle Acceleration and Magnetization}",
  journal = {\ssr},
archivePrefix = "arXiv",
   eprint = {1506.02034},
 primaryClass = "astro-ph.HE",
 keywords = {Acceleration of particles, Galaxies: active, Gamma rays: bursts, Magnetic fields, Pulsars: general, Radiation mechanisms: non-thermal, Relativistic processes},
     year = 2015,
    month = oct,
   volume = 191,
    pages = {519-544},
      doi = {10.1007/s11214-015-0181-8},
   adsurl = {http://adsabs.harvard.edu/abs/2015SSRv..191..519S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kirk_Brian_10,
   author = {{Kirk}, J.~G. and {Reville}, B.},
    title = "{Radiative Signatures of Relativistic Shocks}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1001.0687},
 primaryClass = "astro-ph.HE",
 keywords = {acceleration of particles, gamma-ray burst: general, radiation mechanisms: non-thermal},
     year = 2010,
    month = feb,
   volume = 710,
    pages = {L16-L20},
      doi = {10.1088/2041-8205/710/1/L16},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...710L..16K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tony_13_Escape,
   author = {{Bell}, A.~R. and {Schure}, K.~M. and {Reville}, B. and {Giacinti}, G.
	},
    title = "{Cosmic-ray acceleration and escape from supernova remnants}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1301.7264},
 primaryClass = "astro-ph.HE",
 keywords = {acceleration of particles, magnetic fields, shock waves, cosmic rays, ISM: supernova remnants},
     year = 2013,
    month = may,
   volume = 431,
    pages = {415-429},
      doi = {10.1093/mnras/stt179},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.431..415B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Martins_09,
   author = {{Martins}, S.~F. and {Fonseca}, R.~A. and {Silva}, L.~O. and 
	{Mori}, W.~B.},
    title = "{Ion Dynamics and Acceleration in Relativistic Shocks}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0903.3573},
 primaryClass = "astro-ph.HE",
 keywords = {acceleration of particles, gamma rays: bursts, methods: numerical},
     year = 2009,
    month = apr,
   volume = 695,
    pages = {L189-L193},
      doi = {10.1088/0004-637X/695/2/L189},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...695L.189M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Casse_05,
   author = {{Casse}, F. and {Marcowith}, A.},
    title = "{Astroparticle yield and transport from extragalactic jet terminal shocks}",
  journal = {Astroparticle Physics},
   eprint = {astro-ph/0411395},
 keywords = {13.85.Tp, 95.30.Qd, 05.20.Dd, 41.60.Ap, 25.20.-x},
     year = 2005,
    month = feb,
   volume = 23,
    pages = {31-56},
      doi = {10.1016/j.astropartphys.2004.11.003},
   adsurl = {http://adsabs.harvard.edu/abs/2005APh....23...31C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tony_05,
   author = {{Bell}, A.~R.},
    title = "{The interaction of cosmic rays and magnetized plasma}",
  journal = {\mnras},
 keywords = {acceleration of particles, magnetic fields, plasmas, turbulence, cosmic rays},
     year = 2005,
    month = mar,
   volume = 358,
    pages = {181-187},
      doi = {10.1111/j.1365-2966.2005.08774.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.358..181B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{heproV,
   author = {{Araudo}, A.~T. and {Bell}, A.~R. and {Blundell}, K.~M.},
    title = "{Particle acceleration and magnetic field amplification in hotspots of FR II galaxies: The case study 4C74.26}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1602.07896},
 primaryClass = "astro-ph.HE",
 keywords = {Astrophysics - High Energy Astrophysical Phenomena},
     year = 2016,
    month = feb,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160207896A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kawakatu_16,
   author = {{Kawakatu}, N. and {Kino}, M. and {Takahara}, F.},
    title = "{Evidence for a significant mixture of electron/positron pairs in FRII jets constrained by cocoon dynamics}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1601.00771},
 primaryClass = "astro-ph.HE",
 keywords = {radiation mechanisms: non-thermal, galaxies: individual: Cygnus A, galaxies: individual: 3C 219, galaxies: individual: 3C 223, galaxies: individual: 3C 284},
     year = 2016,
    month = mar,
   volume = 457,
    pages = {1124-1136},
      doi = {10.1093/mnras/stw010},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.457.1124K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tavecchio_05,
   author = {{Tavecchio}, F. and {Cerutti}, R. and {Maraschi}, L. and {Sambruna}, R.~M. and 
	{Gambill}, J.~K. and {Cheung}, C.~C. and {Urry}, C.~M.},
    title = "{X-Ray and Optical Emission from Radio Hot Spots of Powerful Quasars}",
  journal = {\apj},
 keywords = {Galaxies: Active, Galaxies: Quasars: General, X-Rays: Galaxies},
     year = 2005,
    month = sep,
   volume = 630,
    pages = {721-728},
      doi = {10.1086/432371},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...630..721T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Meisenheimer_86_3C33,
   author = {{Meisenheimer}, K. and {Roeser}, H.-J.},
    title = "{Optical synchrotron emission in the southern lobe of 3C33}",
  journal = {\nat},
 keywords = {Optical Emission Spectroscopy, Optical Polarization, Polarimetry, Radio Sources (Astronomy), Synchrotron Radiation, Charge Coupled Devices, Particle Acceleration, Relativistic Electron Beams, Very Large Array (Vla)},
     year = 1986,
    month = feb,
   volume = 319,
    pages = {459-463},
      doi = {10.1038/319459a0},
   adsurl = {http://adsabs.harvard.edu/abs/1986Natur.319..459M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{Ginzburg,
   author = {{Ginzburg}, V.~L. and {Syrovatskii}, S.~I.},
    title = "{The Origin of Cosmic Rays}",
booktitle = {The Origin of Cosmic Rays, New York: Macmillan, 1964},
     year = 1964,
   adsurl = {http://adsabs.harvard.edu/abs/1964ocr..book.....G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Brunetti_97,
   author = {{Brunetti}, G. and {Setti}, G. and {Comastri}, A.},
    title = "{Inverse Compton X-rays from strong FRII radio-galaxies.}",
  journal = {\aap},
   eprint = {astro-ph/9704162},
 keywords = {RADIATION MECHANISM: NON-THERMAL, SCATTERING, GALAXIES: ACTIVE, QUASARS: GENERAL, X-RAYS: GENERAL},
     year = 1997,
    month = sep,
   volume = 325,
    pages = {898-910},
   adsurl = {http://adsabs.harvard.edu/abs/1997A%26A...325..898B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Boccardi_16,
   author = {{Boccardi}, B. and {Krichbaum}, T.~P. and {Bach}, U. and {Mertens}, F. and 
	{Ros}, E. and {Alef}, W. and {Zensus}, J.~A.},
    title = "{The stratified two-sided jet of <ASTROBJ>Cygnus A</ASTROBJ>. Acceleration and collimation}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1509.06250},
 primaryClass = "astro-ph.HE",
 keywords = {galaxies: jets, galaxies: active, instrumentation: high angular resolution},
     year = 2016,
    month = jan,
   volume = 585,
      eid = {A33},
    pages = {A33},
      doi = {10.1051/0004-6361/201526985},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...585A..33B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Boccardi_16Letter,
   author = {{Boccardi}, B. and {Krichbaum}, T.~P. and {Bach}, U. and {Bremer}, M. and 
	{Zensus}, J.~A.},
    title = "{First 3 mm-VLBI imaging of the two-sided jet in Cygnus A. Zooming into the launching region}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1603.04221},
 primaryClass = "astro-ph.HE",
 keywords = {instrumentation: high angular resolution, galaxies: active, galaxies: jets},
     year = 2016,
    month = apr,
   volume = 588,
      eid = {L9},
    pages = {L9},
      doi = {10.1051/0004-6361/201628412},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...588L...9B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Carilli_96,
   author = {{Carilli}, C.~L. and {Perley}, R.~A. and {Bartel}, N. and {Sorathia}, B.
	},
    title = "{The Jets in Cygnus A}",
booktitle = {Energy Transport in Radio Galaxies and Quasars},
     year = 1996,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 100,
   editor = {{Hardee}, P.~E. and {Bridle}, A.~H. and {Zensus}, J.~A.},
    pages = {287},
   adsurl = {http://adsabs.harvard.edu/abs/1996ASPC..100..287C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kino_12,
   author = {{Kino}, M. and {Kawakatu}, N. and {Takahara}, F.},
    title = "{Calorimetry of Active Galactic Nucleus Jets: Testing Plasma Composition in Cygnus A}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1204.3363},
 primaryClass = "astro-ph.HE",
 keywords = {galaxies: individual: Cygnus A, magnetic fields, radiation mechanisms: non-thermal, radio continuum: galaxies, X-rays: galaxies},
     year = 2012,
    month = jun,
   volume = 751,
      eid = {101},
    pages = {101},
      doi = {10.1088/0004-637X/751/2/101},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...751..101K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Harris_94_Xrays,
   author = {{Harris}, D.~E. and {Carilli}, C.~L. and {Perley}, R.~A.},
    title = "{X-ray emission from the radio hotspots of Cygnus A}",
  journal = {\nat},
     year = 1994,
    month = feb,
   volume = 367,
    pages = {713-716},
      doi = {10.1038/367713a0},
   adsurl = {http://adsabs.harvard.edu/abs/1994Natur.367..713H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Leahy_89,
   author = {{Leahy}, J.~P. and {Muxlow}, T.~W.~B. and {Stephens}, P.~W.},
    title = "{151-MHz and 1.5-GHz observations of bridges in powerful extragalactic radio sources}",
  journal = {\mnras},
 keywords = {Astronomical Maps, Extragalactic Radio Sources, Quasars, Radio Astronomy, Radio Galaxies, Angular Distribution, High Resolution, Power Spectra, Radiation Distribution},
     year = 1989,
    month = jul,
   volume = 239,
    pages = {401-440},
      doi = {10.1093/mnras/239.2.401},
   adsurl = {http://adsabs.harvard.edu/abs/1989MNRAS.239..401L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ito_08,
   author = {{Ito}, H. and {Kino}, M. and {Kawakatu}, N. and {Isobe}, N. and 
	{Yamada}, S.},
    title = "{The Estimate of Kinetic Power of Jets in FR II Radio Galaxies: Existence of Invisible Components?}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0807.1946},
 keywords = {galaxies: individual: Cygnus A 3C 223 3C 284 3C 219, radiation mechanisms: non-thermal, radio continuum: galaxies, X-rays: galaxies},
     year = 2008,
    month = oct,
   volume = 685,
      eid = {828-838},
    pages = {828-838},
      doi = {10.1086/591036},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...685..828I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kino_04,
   author = {{Kino}, M. and {Takahara}, F.},
    title = "{Constraints on the energetics and plasma composition of relativistic jets in FR II sources}",
  journal = {\mnras},
   eprint = {astro-ph/0312530},
 keywords = {acceleration of particles, radiation mechanisms: non-thermal, galaxies: active},
     year = 2004,
    month = mar,
   volume = 349,
    pages = {336-346},
      doi = {10.1111/j.1365-2966.2004.07511.x},
   adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.349..336K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cutoff_nrh,
   author = {{Araudo}, A.~T. and {Bell}, A.~R. and {Crilly}, A. and {Blundell}, K.~M.
	},
    title = "{Evidence that the maximum electron energy in hotspots of FR II galaxies is not determined by synchrotron cooling}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1605.05125},
 primaryClass = "astro-ph.HE",
 keywords = {galaxies: active, galaxies: jets, acceleration of particles, radiation mechanisms: non-thermal, shock waves},
     year = 2016,
    month = may,
      doi = {10.1093/mnras/stw1204},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.tmp..889A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CygA_gammamin,
   author = {{McKean}, J.~P. and {Godfrey}, L.~E.~H. and {Vegetti}, S. and 
	{Wise}, M.~W. and {Morganti}, R. and {Hardcastle}, M.~J. and 
	{Rafferty}, D. and {Anderson}, J. and {Avruch}, I.~M. and {Beck}, R. and 
	{Bell}, M.~E. and {van Bemmel}, I. and {Bentum}, M.~J. and {Bernardi}, G. and 
	{Best}, P. and {Blaauw}, R. and {Bonafede}, A. and {Breitling}, F. and 
	{Broderick}, J.~W. and {Br{\"u}ggen}, M. and {Cerrigone}, L. and 
	{Ciardi}, B. and {de Gasperin}, F. and {Deller}, A. and {Duscha}, S. and 
	{Engels}, D. and {Falcke}, H. and {Fallows}, R.~A. and {Frieswijk}, W. and 
	{Garrett}, M.~A. and {Grie{\ss}meier}, J.~M. and {van Haarlem}, M.~P. and 
	{Heald}, G. and {Hoeft}, M. and {Horst}, A.~J.~v.~d. and {Iacobelli}, M. and 
	{Intema}, H. and {Juette}, E. and {Karastergiou}, A. and {Kondratiev}, V.~I. and 
	{Koopmans}, L.~V.~E. and {Kuniyoshi}, M. and {Kuper}, G. and 
	{van Leeuwen}, J. and {Maat}, P. and {Mann}, G. and {Markoff}, S. and 
	{McFadden}, R. and {McKay-Bukowski}, D. and {Mulcahy}, D.~D. and 
	{Munk}, H. and {Nelles}, A. and {Orru}, E. and {Paas}, H. and 
	{Pandey-Pommier}, M. and {Pietka}, M. and {Pizzo}, R. and {Polatidis}, A.~G. and 
	{Reich}, W. and {R{\"o}ttgering}, H.~J.~A. and {Rowlinson}, A. and 
	{Scaife}, A.~M.~M. and {Serylak}, M. and {Shulevski}, A. and 
	{Sluman}, J. and {Smirnov}, O. and {Steinmetz}, M. and {Stewart}, A. and 
	{Swinbank}, J. and {Tagger}, M. and {Thoudam}, S. and {Toribio}, M.~C. and 
	{Vermeulen}, R. and {Vocks}, C. and {van Weeren}, R.~J. and 
	{Wucknitz}, O. and {Yatawatta}, S. and {Zarka}, P.},
    title = "{LOFAR imaging of Cygnus A - direct detection of a turnover in the hotspot radio spectra}",
  journal = {\mnras},
 keywords = {radio continuum: galaxies},
     year = 2016,
    month = dec,
   volume = 463,
    pages = {3143-3150},
      doi = {10.1093/mnras/stw2105},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.463.3143M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Riquelme_10,
   author = {{Riquelme}, M.~A. and {Spitkovsky}, A.},
    title = "{Magnetic Amplification by Magnetized Cosmic Rays in Supernova Remnant Shocks}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0912.4990},
 primaryClass = "astro-ph.HE",
 keywords = {cosmic rays, ISM: jets and outflows, ISM: magnetic fields, ISM: supernova remnants},
     year = 2010,
    month = jul,
   volume = 717,
    pages = {1054-1066},
      doi = {10.1088/0004-637X/717/2/1054},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...717.1054R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wilson_06,
   author = {{Wilson}, A.~S. and {Smith}, D.~A. and {Young}, A.~J.},
    title = "{The Cavity of Cygnus A}",
  journal = {\apjl},
   eprint = {astro-ph/0603435},
 keywords = {Galaxies: Active, Galaxies: Clusters: General, Galaxies: Individual: Name: Cygnus A, Galaxies: Jets, Galaxies: Nuclei, X-Rays: Galaxies},
     year = 2006,
    month = jun,
   volume = 644,
    pages = {L9-L12},
      doi = {10.1086/504108},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...644L...9W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rachen_93,
   author = {{Rachen}, J.~P. and {Biermann}, P.~L.},
    title = "{Extragalactic Ultra-High Energy Cosmic-Rays - Part One - Contribution from Hot Spots in Fr-II Radio Galaxies}",
  journal = {\aap},
   eprint = {astro-ph/9301010},
     year = 1993,
    month = may,
   volume = 272,
    pages = {161},
   adsurl = {http://adsabs.harvard.edu/abs/1993A%26A...272..161R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Norman_95,
   author = {{Norman}, C.~A. and {Melrose}, D.~B. and {Achterberg}, A.},
    title = "{The Origin of Cosmic Rays above 10 18.5 eV}",
  journal = {\apj},
 keywords = {ACCELERATION OF PARTICLES, ISM: COSMIC RAYS, SHOCK WAVES},
     year = 1995,
    month = nov,
   volume = 454,
    pages = {60},
      doi = {10.1086/176465},
   adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...454...60N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ostrowski_02,
   author = {{Ostrowski}, M. and {Bednarz}, J.},
    title = "{Comment on the first-order Fermi acceleration at ultra-relativistic shocks}",
  journal = {\aap},
   eprint = {astro-ph/0101069},
 keywords = {acceleration of particles, shock waves, X-rays: bursts, gamma-rays: bursts, ISM: cosmic rays},
     year = 2002,
    month = nov,
   volume = 394,
    pages = {1141-1144},
      doi = {10.1051/0004-6361:20021173},
   adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...394.1141O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tony_escape_13,
   author = {{Bell}, A.~R. and {Schure}, K.~M. and {Reville}, B. and {Giacinti}, G.
	},
    title = "{Cosmic-ray acceleration and escape from supernova remnants}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1301.7264},
 primaryClass = "astro-ph.HE",
 keywords = {acceleration of particles, magnetic fields, shock waves, cosmic rays, ISM: supernova remnants},
     year = 2013,
    month = may,
   volume = 431,
    pages = {415-429},
      doi = {10.1093/mnras/stt179},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.431..415B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{James_17,
   author = {{Matthews}, J.~H. and {Bell}, A.~R. and {Blundell}, K.~M. and 
	{Araudo}, A.~T.},
    title = "{Amplification of perpendicular and parallel magnetic fields by cosmic ray currents}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1704.02985},
 primaryClass = "astro-ph.HE",
 keywords = {acceleration of particles, magnetic fields, MHD, turbulence, ISM: supernova remnants, galaxies: jets},
     year = 2017,
    month = aug,
   volume = 469,
    pages = {1849-1860},
      doi = {10.1093/mnras/stx905},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.469.1849M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Orienti_17,
   author = {{Orienti}, M. and {Brunetti}, G. and {Nagai}, H. and {Paladino}, R. and 
	{Mack}, K.-H. and {Prieto}, M.~A.},
    title = "{ALMA polarization observations of the particle accelerators in the hot spot of the radio galaxy 3C 445}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1705.06465},
 primaryClass = "astro-ph.HE",
 keywords = {Astrophysics - High Energy Astrophysical Phenomena},
     year = 2017,
    month = may,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170506465O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Owen_97,
   author = {{Owen}, F.~N. and {Ledlow}, M.~J. and {Morrison}, G.~E. and 
	{Hill}, J.~M.},
    title = "{The Cluster of Galaxies Surrounding Cygnus A}",
  journal = {\apjl},
   eprint = {astro-ph/9708150},
 keywords = {GALAXIES: ACTIVE, GALAXIES: DISTANCES AND REDSHIFTS, GALAXIES: INDIVIDUAL NAME: CYGNUS A, GALAXIES: CLUSTERS: INDIVIDUAL NAME: CYGNUS A, Galaxies: Active, Galaxies: Clusters: Individual: Name: Cygnus A, Galaxies: Distances and Redshifts, Galaxies: Individual: Name: Cygnus A},
     year = 1997,
    month = oct,
   volume = 488,
    pages = {L15-L17},
      doi = {10.1086/310908},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...488L..15O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Tony_17,
   author = {{Bell}, A. and {Araudo}, A. and {Matthews}, J. and {Blundell}, K.
	},
    title = "{Cosmic Ray Acceleration by Relativistic Shocks: Limits and Estimates}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1709.07793},
 primaryClass = "astro-ph.HE",
 keywords = {Astrophysics - High Energy Astrophysical Phenomena},
     year = 2017,
    month = sep,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170907793B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

